Les Houches 2015: Physics at TeV Colliders Standard Model Working Group Report

This Report summarizes the proceedings of the 2015 Les Houches workshop on Physics at TeV Colliders. Session 1 dealt with (I) new developments relevant for high precision Standard Model calculations, (II) the new PDF4LHC parton distributions, (III) issues in the theoretical description of the production of Standard Model Higgs bosons and how to relate experimental measurements, (IV) a host of phenomenological studies essential for comparing LHC data from Run I with theoretical predictions and projections for future measurements in Run II, and (V) new developments in Monte Carlo event generators.

==> dyew_main.tex <==
\section{Electroweak corrections in Drell--Yan production
  \texorpdfstring{\protect\footnote{ A.\ Huss, M.\ Sch\"onherr}}{}}

\subsection{Introduction}
\label{sec:dyew:intro}

%%%%% Motivation -> neutral-current DY
The Drell--Yan-like production of electroweak gauge bosons represents one of the key Standard Model processes at hadron colliders whose detailed understanding is crucial in order to exploit the full potential of the measurements performed at the LHC.
The neutral-current process $\mathrm{p}\mathrm{p}\to\mathrm{Z}/\gamma\to\ell^+\ell^-$, in particular, has a very clean experimental signature owing to the two charged leptons in the final state which further allows for the full reconstruction of the kinematics of the intermediate gauge boson.
Not only does this process constitute a powerful tool for detector calibration, but it also delivers important constraints in the fit of PDFs and allows for precision measurements such as the extraction of the weak mixing angle $\sin^2(\theta^{\ell}_\mathrm{eff})$.

%%%%% Theory status: fixed order
On the theory side, Drell--Yan production belongs to one of the most precisely predicted processes:
QCD corrections are known up to NNLO~~\cite{Hamberg:1990np,Harlander:2002wh,Anastasiou:2003ds,Melnikov:2006di,Melnikov:2006kv,Catani:2009sm,Gavin:2010az,Gavin:2012sy}, the electroweak~(EW) corrections up to NLO~\cite{Baur:1997wa,Zykunov:2001mn,Baur:2001ze,Dittmaier:2001ay,Baur:2004ig,Arbuzov:2005dd,CarloniCalame:2006zq,Zykunov:2005tc,CarloniCalame:2007cd,Arbuzov:2007db,Brensing:2007qm,Dittmaier:2009cr}, and many further improvements beyond fixed-order predictions (see, e.g., references in Ref.~\cite{Dittmaier:2015rxo}).
Until recently, the largest missing piece in terms of fixed-order predictions were given by the NNLO mixed QCD--EW corrections.
Different approaches of combining QCD and EW corrections revealed that the missing $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections could have an impact of a few per cent in the resonance region, i.e.\ at the level that is relevant for precision phenomenology.
In a series of papers~\cite{Dittmaier:2014qza,Dittmaier:2015rxo}, the calculation of these corrections have been tackled using the so-called pole approximation~(PA).
This approach is suitable to describe observables that are dominated by resonances with sufficient accuracy.

%%%%% Some context
In this work, we investigate how the $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections 
generated through a universal process-independent resummation approach 
compares to the results of Ref.~\cite{Dittmaier:2015rxo}.
Section~\ref{sec:dyew:comp} gives a brief overview of the computation 
employing the PA and the implementation of the QED shower in the 
\textsc{Sherpa} Monte Carlo program~\cite{Gleisberg:2008ta}.
In Sect.~\ref{sec:dyew:results} we present our numerical results of the 
comparison before we conclude in Sect.~\ref{sec:dyew:conclusions}.


\subsection{Computational setup}
\label{sec:dyew:comp}

%%%%% The pole approximation
\paragraph*{The Pole approximation}
The calculation of the $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections presented in Refs.~\cite{Dittmaier:2014qza,Dittmaier:2015rxo} was performed in the framework of a pole expansion, which is based on a systematic expansion of the cross section around the gauge-boson resonance $p_V^2\sim\mu_V^2$, with $\mu_V^2=M_V^2-\mathrm{i} M_V\Gamma_V$ denoting the gauge-invariant location of the propagator pole in the complex plane. 
Only retaining the leading contributions that are enhanced by a resonant propagator, we obtain the so-called pole approximation~(PA).
As a result of applying the PA, the calculation is split into separate well-defined parts that can be classified into the non-factorizable and factorizable corrections: 
The non-factorizable corrections involve soft-photon exchange between the production and decay stages of the process and constitute the conceptually most difficult part of the calculation.
They have been computed in Ref.~\cite{Dittmaier:2014qza} and were found to be negligible for all phenomenological purposes.
The factorizable contributions, on the other hand, involve corrections where the production of the intermediate gauge boson and its decay proceed independently. 
Here, the factorizable corrections of ``initial--final'' type were identified as the numerically dominant contribution---combining the sizeable QCD corrections to the production sub-process with the large EW corrections of the gauge boson decay---and were computed in Ref.~\cite{Dittmaier:2015rxo}.
The remaining factorizable corrections are given by the ``initial--initial'' and ``finial--final'' types.
The latter were found to be numerically negligible~\cite{Dittmaier:2015rxo}, while the former are not expected to deliver a sizeable correction, in particular for observables that are less sensitive to initial-state radiation effects.
In the remainder of this work, we will thus focus our attention to the initial--final factorizable corrections which we will often simply refer to as the $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections in the PA.
More details on this calculation can be found in Refs.~\cite{Dittmaier:2014qza,Dittmaier:2015rxo}.

%%%%% Sherpa's YFS shower
\paragraph*{The QED resummation in Sherpa}
Another approach to higher order QED or electroweak corrections is 
presented in the soft-photon resummation of Yennie, Frautschi and 
Suura (YFS)~\cite{Yennie:1961ad}. Therein the universal structure 
of real and virtual soft photon emissions is exploited to construct 
an all-order approximation to the process at hand which can be 
systematically supplemented with process-dependent finite hard 
real and virtual emission corrections. The implementation presented 
in Ref.~\cite{Schonherr:2008av} focusses on higher-order QED corrections 
to particle decays and is used since as the default mechanism for such 
corrections in \textsc{Sherpa}~\cite{Gleisberg:2008ta}, both for 
elementary particle (e.g.\ $\mathrm{W}^{\pm}$, $\mathrm{Z}$, $\tau^\pm$) as well as 
hadron decays. 

In the present context of lepton pair production the higher-order 
QED corrections are effected in a factorised approach. The complete 
process $\mathrm{p}\mathrm{p}\to\ell^+\ell^-$ is calculated at LO or NLO in the strong 
coupling constant keeping all off-shell effects. Then, an intermediate 
resonance $X$ is reconstructed from the lepton pair and assigned its 
invariant mass. Its decay width is then corrected for higher order 
QED corrections, including YFS resummation, to 
\begin{equation}
  \begin{split}\label{eq:dyew:comp:yfs}
    \Gamma
    \,=\;&
      \frac{1}{2m_X}\sum\limits_{n_\gamma=0}^\infty\frac{1}{n_\gamma !}
      \int\mathrm{d}\Phi\;\mathrm{e}^{Y(\Omega)}
      \prod\limits_{i=1}^{n_\gamma}\mathrm{d}\Phi_i\,\tilde{S}(k_i)\,\Theta(k_i,\Omega)
      \left[
        \tilde\beta_0^0
        +\tilde\beta_0^1
        +\sum\limits_{i=1}^{n_\gamma}\frac{\tilde\beta_1^1(k_i)}{\tilde{S}(k_i)}
        +\mathcal{O}(\alpha^2)
      \right]\;.
  \end{split}
\end{equation}
Therein, $m_X$ is the mass of the decaying resonance and $\mathrm{d}\Phi$ 
is the phase element of the leading order decay, and $\tilde\beta_0^0$ is 
the leading order decay squared matrix element. The $Y(\Omega)$ then 
is the sum of the eikonal approximations to virtual photon exchange and 
unresolved soft real photon emission, $\Omega$ denoting the region in which 
soft photons are not resolvable. The YFS form factor, $\mathrm{e}^{Y(\Omega)}$, then 
resums these leading logarithmic universal corrections to all orders. 
Resolved photons are then described explicitly, emission by emission, 
by the eikonal $\tilde{S}$ depending on the individual photon momentum 
$k_i$. $\mathrm{d}\Phi_i$ is the corresponding phase space element. The 
eikonal approximations used in both the YFS form factor and for 
resolved real emissions can then, order-by-order, be corrected by 
supplementing the corresponding infrared-subtracted squared matrix 
elements $\tilde\beta_i^{i+j}$ of $\mathcal{O}(\alpha^{i+j})$ relative to 
the Born decay and containing $i$ resolved photons. Since all charged 
particles are considered massive in the context of YFS resummation, 
all $\tilde\beta_i$ are free of any infrared singularity. Finally, it is 
interesting to note that in the case of multi-photon emission 
each emitted photon receives the hard emission correction $\tilde\beta_1^1$ 
in the respective one-photon emission projected phase space.

The implementation used here, as we restrict the $\gamma^*/Z$ propagator 
virtuality to be near the $Z$ mass, always identifies the resonance $X$ with 
the $Z$ boson. The calculation thus contains the $\mathcal{O}(\alpha)$ virtual 
corrections $\tilde\beta_0^1$ and real emission corrections $\tilde\beta_1^1$ 
resulting in an NLO QED accurate description. As NLO weak corrections 
are finite they can in principle be incorporated in the $\tilde\beta_0^1$. 
This is left to a future work.


\subsection{Results}
\label{sec:dyew:results}

%%%%% numerical setup
The numerical results presented in this section are obtained using 
the same input parameters and event selection cuts as in 
Ref.~\cite{Dittmaier:2015rxo}. The electroweak coupling constant 
$\alpha$ is defined in the $G_\mu$-scheme, with the exception of 
the photonic corrections which use $\alpha(0)$ as their coupling. 
For the parton distribution functions we use the NNPDF2.3QED NLO PDF 
set~\cite{Ball:2012cx}, in particular also the LO predictions shown in 
the following were evaluated using this choice. For the charged 
leptons in the final state we consider two different reconstruction 
strategies: In the case of ``dressed'' electrons, we apply a photon 
recombination procedure in order to treat all collinear 
lepton--photon configurations inclusively, whereas in the ``bare'' 
muon setup no such recombination is performed. Further details on 
the calculational setup and the event reconstruction are given in 
Ref.~\cite{Dittmaier:2015rxo}.

%%%%% define delta
In order to establish the setup of the two computations, we first 
consider the relative $\mathcal{O}(\alpha)$ corrections by applying 
the YFS resummation in \textsc{Sherpa} to the LO prediction, 
$\sigma^{\mathrm{LO}\otimes\mathrm{YFS}}$, and compare it to the full 
EW corrections denoted as $\sigma^{\mathrm{NLO}[\mathrm{EW}]}$%
\footnote{
  A comparison of the PA at $\mathcal{O}(\alpha)$ against the full 
  NLO EW corrections has been performed in Ref.~\cite{Dittmaier:2014qza}.
}.
The respective relative correction factors, normalised to the LO 
prediction, are then given by
\begin{align}
  \label{eq:dyew:delta:nlo}
  \delta_\alpha^\mathrm{YFS} &= 
  \frac{\sigma^{\mathrm{LO}\otimes\mathrm{YFS}} - \sigma^\mathrm{LO}}{\sigma^\mathrm{LO}}
  , &
  \delta_\alpha &= 
  \frac{\sigma^{\mathrm{NLO}[\mathrm{EW}]} - \sigma^\mathrm{LO}}{\sigma^\mathrm{LO}}
  .
\end{align}
Please note, the thus defined $\delta_\alpha^\mathrm{YFS}$ retains also 
higher orders of $\alpha$ contrary to $\delta_\alpha$. For the 
mixed QCD--EW corrections, we generate terms of $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ 
by applying the YFS resummation on top of the fixed-order NLO QCD 
prediction, which we denote by $\sigma^{\mathrm{NLO}[\mathrm{QCD}]\otimes\mathrm{YFS}}$.
These results are compared to the best prediction of 
Ref.~\cite{Dittmaier:2015rxo}, $\sigma^{\mathrm{NNLO}[\mathrm{QCD}\times\mathrm{EW}]}_{\mathrm{PA}}$, 
which includes the full NLO QCD and EW corrections, supplemented by 
the dominant $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections in the PA. In order 
to extract the genuine $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ contribution from the 
prediction based on the YFS resummation, we define the relative 
correction factor as follows,
\begin{align}
  \label{eq:dyew:delta:nnlo:yfs}
  \delta_{\alpha_\mathrm{s}\alpha}^\mathrm{YFS} &= 
  \frac{ (\sigma^{\mathrm{NLO}[\mathrm{QCD}]\otimes\mathrm{YFS}} - \sigma^{\mathrm{NLO}[\mathrm{QCD}]}) 
        -(\sigma^{\mathrm{LO}\otimes\mathrm{YFS}} - \sigma^\mathrm{LO})}
       {\sigma^\mathrm{LO}} .
\end{align}
For the fixed-order prediction in the PA, the corresponding correction 
factor is given by
\begin{align}
  \label{eq:dyew:delta:nnlo:pa}
  \delta_{\alpha_\mathrm{s}\alpha}^\mathrm{PA} &= 
    \frac{\sigma^{\mathrm{NNLO}[\mathrm{QCD}\times\mathrm{EW}]}_{\mathrm{PA}} - \sigma^{\mathrm{NLO}[\mathrm{QCD}+\mathrm{EW}]}}
       {\sigma^\mathrm{LO}} .
\end{align}
Again, as in Eq.~\ref{eq:dyew:delta:nlo}, $\delta_{\alpha_\mathrm{s}\alpha}^\mathrm{YFS}$ 
also contains higher orders in $\alpha$, contrary to 
$\delta_{\alpha_\mathrm{s}\alpha}^\mathrm{PA}$.

%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \includegraphics[width=.48\linewidth]{images/Z_mll2_LO.pdf} \hfill
  \includegraphics[width=.48\linewidth]{images/Z_mll2_NLO.pdf} 
  \caption{
    Comparison of the $\mathcal{O}(\alpha)$~(left) and $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ 
    (right) corrections to the invariant-mass distribution of the lepton 
    pair $m_{\ell\ell}$ between Ref.~\cite{Dittmaier:2015rxo} and Sherpa. 
    The absolute distributions and the relative corrections at the 
    respective order are shown in the top and bottom panels, respectively. 
    Collinear lepton--photon configurations are treated both inclusively 
    with a recombination procedure resulting in the ``e dressed'' setup 
    (blue) or exclusively in the case of muons labelled as ``$\mu$ bare'' 
    (red).
  }
  \label{fig:dyew:mll}
\end{figure}
%%%%%
\begin{figure}
  \includegraphics[width=.48\linewidth]{images/Z_ptl+2_LO.pdf} \hfill
  \includegraphics[width=.48\linewidth]{images/Z_ptl+2_NLO.pdf} 
  \caption{
    Comparison of the $\mathcal{O}(\alpha)$~(left) and $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ 
    (right) corrections to the transverse-momentum distribution of the 
    positively charged lepton $p_\mathrm{T}^{\ell^+}$ between 
    Ref.~\cite{Dittmaier:2015rxo} and Sherpa. The absolute distributions 
    and the relative corrections at the respective order are shown in the 
    top and bottom panels, respectively. Collinear lepton--photon 
    configurations are treated both inclusively with a recombination 
    procedure resulting in the ``e dressed'' setup~(blue) or exclusively in 
    the case of muons labelled as ``$\mu$ bare''~(red).
  }
  \label{fig:dyew:ptl}
\end{figure}
%%%%%
\begin{figure}
  \includegraphics[width=.48\linewidth]{images/Z_yll_LO.pdf} \hfill
  \includegraphics[width=.48\linewidth]{images/Z_yll_NLO.pdf}
  \caption{
    Comparison of the $\mathcal{O}(\alpha)$~(left) and $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ 
    (right) corrections to the rapidity distribution of the lepton pair 
    $y_{\ell\ell}$ between Ref.~\cite{Dittmaier:2015rxo} and Sherpa. The 
    absolute distributions and the relative corrections at the respective 
    order are shown in the top and bottom panels, respectively. Collinear 
    lepton--photon configurations are treated both inclusively with a 
    recombination procedure resulting in the ``e dressed'' setup~(blue) or 
    exclusively in the case of muons labelled as ``$\mu$ bare''~(red).
  }
  \label{fig:dyew:yll}
\end{figure}
%%%%%%%%%%%%%%%%%%%%


%%%%% discuss results
The numerical results comprise differential distributions in the 
lepton invariant mass $m_{\ell\ell}$, the transverse momentum of the 
positively charged lepton $p_\mathrm{T}^{\ell^+}$, and the rapidity of the 
lepton pair $y_{\ell\ell}$, which are shown in 
Figs.~\ref{fig:dyew:mll}--\ref{fig:dyew:yll}, respectively. The left plot 
in the figures shows a comparison of the $\mathcal{O}(\alpha)$ corrections, 
while the right-hand plot compares the corresponding $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ 
corrections. In each plot we show the absolute distributions in 
the top frame and the relative correction factors in the bottom 
panel as defined in Eq.~\eqref{eq:dyew:delta:nlo} for the $\mathcal{O}(\alpha)$ 
and Eqs.~\eqref{eq:dyew:delta:nnlo:yfs} and \eqref{eq:dyew:delta:nnlo:pa} 
for the mixed QCD--EW corrections.

%% mll
For the invariant mass distribution shown in Fig.~\ref{fig:dyew:mll} we 
observe an overall good agreement between the YFS resummation and 
the fixed-order result. This reflects the property of this observable 
whose corrections are known to be dominated by final-state photon 
emission. Both at $\mathcal{O}(\alpha)$ and $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ we 
observe a small offset between the two predictions where the resummed 
approach leads to slightly smaller corrections below the $\mathrm{Z}$ 
resonance. This difference originates from multi-photon emissions, 
which is included in the YFS formalism, cf.\ Eq.~\eqref{eq:dyew:comp:yfs}, 
whereas the fixed-order prediction is restricted to at most one 
photon emission.
%% ptlp
Figure~\ref{fig:dyew:ptl} shows the corrections to the transverse momentum 
distribution of the positively charged lepton, $p_\mathrm{T}^{\ell^+}$. Although 
qualitatively displaying a similar shape in the $\mathcal{O}(\alpha)$ corrections, 
we observe larger differences between the two computations around the 
resonance and in the higher transverse momentum tails. This difference 
can be understood from the fact that this observable is sensitive to 
recoil effects from initial-state radiation which are not accounted for 
in the YFS approach as used here.  Indeed, comparing the final-state 
factorizable $\mathcal{O}(\alpha)$ corrections in PA to the full NLO EW 
corrections, as it is done in Fig.~9 in Ref.~\cite{Dittmaier:2014qza},
a very similar behaviour can be observed.
For the mixed QCD--EW corrections, on 
the other hand, the EW corrections contained in the 
$\mathcal{O}(\alpha_\mathrm{s}\alpha)$ PA prediction are confined to the decay 
sub-process similarly to the case of the YFS resummation. As a result, 
we see a much better agreement between the two computations here.
%% yll
Lastly, the numerical results for the rapidity distribution of the 
lepton pair, $y_{\ell\ell}$, are shown in Fig.~\ref{fig:dyew:yll}. At 
$\mathcal{O}(\alpha)$, the resummed prediction is able to reproduce the 
exact fixed-order result to a large extent up to a small offset in 
the normalisation. This shift can be attributed to the finite weak 
corrections which are missing in the YFS resummed prediction here. 
The purely weak corrections amount to a flat correction of 
approximately $-0.5\%$ in this distribution as can be read off from
Fig.~14 in Ref.~\cite{Dittmaier:2009cr} and matches well with 
the observed offset. For the mixed QCD--EW corrections we obtain 
corrections from the YFS resummation that are similar in shape to 
those of the fixed-order prediction in the PA, however, with larger 
negative corrections in the forward regime which possibly stem from 
multi-photon effects on the event acceptance in this region.



\subsection{Conclusions and outlook}
\label{sec:dyew:conclusions}

%%%%% short summary
The Drell--Yan process is one of the most important ``standard candle'' 
processes at the LHC and, as such, has a wide range of applications.
In this work, we have explored the possibility of generating mixed 
QCD--EW corrections of $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ to this process using 
the YFS resummation available in the \textsc{Sherpa} Monte Carlo and 
performed a comparison to the fixed-order calculation of 
Ref.~\cite{Dittmaier:2015rxo}. To this end, we have considered both 
$\mathcal{O}(\alpha)$ and $\mathcal{O}(\alpha_\mathrm{s}\alpha)$ corrections to various 
differential distributions given by the invariant mass of the leptons, 
the lepton transverse momentum, and the rapidity of the lepton pair.
We find that the QED resummation is able to capture the electroweak 
corrections to these observables remarkably well.
Furthermore, we were able to identify various sources for the differences 
that were observed between the two predictions.

%%%%% outlook
Building on the insights that were gained from this study, it will 
be interesting to investigate further observables and also repeating 
this comparison for the charged-current process. Potential 
improvements were identified in both computations which should be 
explored in order to gain further insights into the numerical impact of 
the various ingredients that enter the two predictions. Such 
improvements include the finite weak corrections that can be 
incorporated to the YFS approach through the $\tilde{\beta}^1$ 
coefficient in Eq.~\eqref{eq:dyew:comp:yfs} on the one side, and 
supplementing the fixed-order calculation with multi-photon emission 
effects. 


\subsection*{Acknowledgements}

We would like to thank the Les Houches workshop for hospitality offered 
during which some of the work contained herein was performed. 
A.H. acknowledges support from the ERC Advanced Grant MC@NNLO (340983). 
MS acknowledges support by the Swiss National Science Foundation (SNF) 
under contract PP00P2-128552.



==> ntuples_main.tex <==
\section{Ntuples for NNLO events produced by \texorpdfstring{\texttt{EERAD3}}{EERAD3} \texorpdfstring{\protect\footnote{ G.~Heinrich, D.~Ma{\^i}tre}}{}}
\label{sec:NNLOntuples}

We study the production of Ntuples based on the program {\tt EERAD3}
which produces parton-level QCD events to calculate event shapes and
jet rates in electron-positron annihilation through to order $\alpha_s^3$.
The aim of this study is to assess the viability of Ntuples as a general
way to have NNLO results stored and made available to the experimental community.

\subsection{Introduction}

High precision calculations will be vital in the next phase(s) of the LHC
in order to be able profit from the high quality data being collected.
In order to further explore the Higgs sector and distinguish
BSM effects from higher order effects within the Standard model,
next-to-next-to leading order (NNLO) predicitions
are necessary for a number of proccesses.
However, such predictions are the results of complex calculations,
which may take a considerable amount of time and computing resources.
Running such programs for various scale choices, parton distribution functions
and sets of cuts  is a tedious, time consuming task.

For processes with multi-particle final states at NLO, one is faced with similar
problems.
A possible solution, described in detail in Ref.~\cite{Bern:2013zja},
is to store the phase space points and the corresponding matrix elememt weights,
together with other relevant information,
in {\tt Root Ntuple} files.
This has the following advantages:
\begin{enumerate}
\item the results are flexible for (tighter) cuts to be applied at a later stage,
\item scale and PDF variations can be performed without lengthy runs of  the original program,
\item it allows to make the results readily available to experimantalists.
\end{enumerate}
The Ntuple format for NLO results already has been used successfully for various
high-multiplicity processes, e.g. W+4\,jets~\cite{Bern:2011ep},
W+5\,jets~\cite{Bern:2013gka}, or H+3\,jets~\cite{Cullen:2013saa,Greiner:2015jha}.

In this note we investigate whether the Ntuple format is also a viable option to store NNLO
results. The limitation here can come only from the size of the files containing the Ntuples.
Total sizes of the order of a TeraByte have proven practical for NLO calculations.


To get a first idea of the file sizes needed to store events which allow to produce reasonably smooth
histograms for observables calculated at NNLO, we take the program {\tt EERAD3}~\cite{Ridder:2014wza} as an example.
{\tt EERAD3} is a parton level event generator which computes the QCD corrections
to event shape observables  and
jet rates in electron-positron annihilation to order $\alpha_s^3$~\cite{GehrmannDeRidder:2007hr,GehrmannDeRidder:2008ug}.
As this example does not require any parton distribution functions, and therefore
does not contain any factorization scale dependence,
it lends itself for a first study,
which can be extended to the case of hadronic collisions later.

\subsection{Ntuples at NNLO}

\subsubsection{Brief description of the {\tt EERAD3} program}

The perturbative expansion for the distribution of an
event shape observable $\Obs$ up to NNLO at the centre-of-mass energy $\sqrt{s}$
and renormalisation scale $\mu^2 = s$, with
$\alpha_s\equiv \alpha_s(\sqrt s)$,  is given by
\begin{eqnarray}
\frac{1}{\sigma_{{\rm had}}}\, \frac{\dbox\sigma}{\dbox \Obs} &=&
\left(\frac{\alpha_s}{2\pi}\right) \frac{\dbox \bar A}{\dbox \Obs} +
\left(\frac{\alpha_s}{2\pi}\right)^2 \frac{\dbox \bar B}{\dbox \Obs}
+ \left(\frac{\alpha_s}{2\pi}\right)^3
\frac{\dbox \bar C}{\dbox \Obs} + {\cal O}(\alpha_s^4)\;.
\label{eq:NNLO}
\end{eqnarray}
In Eq.~(\ref{eq:NNLO}) the event shape distribution
is normalised to the total hadronic cross section $\sigma_{\rm{had}}$.
The latter can be expanded as
\begin{equation}
  \sigma_{\rm{had}}=\sigma_0\,
\left(1+\frac{3}{2}C_F\,\left(\frac{\alpha_s}{2\pi}\right)
+K_2\,\left(\frac{\alpha_s}{2\pi}\right)^2+{\cal O}(\alpha_s^3)\,
\right) \;,
\end{equation}
where the Born cross section for $e^+e^- \to q \bar q$ is
$\sigma_0 = \frac{4 \pi \alpha}{3 s} N  e_q^2$,
assuming massless quarks.
The constant $K_2$ is given by~\cite{Chetyrkin:1996ia}
\begin{equation}
  K_2=\frac{1}{4}\left[- \frac{3}{2}C_F^2
+C_FC_A\,\left(\frac{123}{2}-44\zeta_3\right)+C_FT_RN_F\,(-22+16\zeta_3)
 \right] \;,
\end{equation}
with
$C_A = N$, $C_F = (N^2-1)/(2N)$,
$T_R = {1}/{2}$,  and $N_F$ light quark flavours.
The program {\tt EERAD3} computes the perturbative coefficients $A$, $B$ and $C$, which are
normalised to $\sigma_0$:
\begin{eqnarray}
\frac{1}{\sigma_0}\, \frac{\dbox\sigma}{d \Obs} &=&
\left(\frac{\alpha_s}{2\pi}\right) \frac{\dbox  A}{\dbox \Obs} +
\left(\frac{\alpha_s}{2\pi}\right)^2 \frac{\dbox  B}{\dbox \Obs}
+ \left(\frac{\alpha_s}{2\pi}\right)^3
\frac{\dbox  C}{\dbox \Obs} + {\cal O}(\alpha_s^4)\,.
\label{eq:NNLOsigma0}
\end{eqnarray}
$A$, $B$ and $C$ are straightforwardly related to $\bar{A}$, $\bar{B}$
and $\bar{C}$:
\begin{eqnarray}
&&\bar{A} = A\;,\;
\bar{B} = B - \frac{3}{2}C_F\,A\;,\;
\bar{C} = C -  \frac{3}{2}C_F\,B+ \left(\frac{9}{4}C_F^2\,-K_2\right)\,A
\;.\label{eq:ceff}
\end{eqnarray}
As these coefficients are computed at a renormalisation scale fixed to
the centre-of-mass energy, they
depend only on the value of the observable $\Obs$.

The QCD coupling constant evolves according to the renormalisation group
equation, which reads to NNLO:
\begin{equation}
\label{eq:running}
\mu^2 \frac{\dbox \alpha_s(\mu)}{\dbox \mu^2} = -\alpha_s(\mu)
\left[\beta_0 \left(\frac{\alpha_s(\mu)}{2\pi}\right)
+ \beta_1 \left(\frac{\alpha_s(\mu)}{2\pi}\right)^2
+ \beta_2 \left(\frac{\alpha_s(\mu)}{2\pi}\right)^3
+ {\cal O}(\alpha_s^4) \right]\,
\end{equation}
The coefficients $\beta_i$ can be found e.g. in \cite{Ridder:2014wza}.
%with the following  coefficients in the $\overline{{\rm MS}}$-scheme:
%\begin{eqnarray}
%\beta_0 &=& \frac{11 \CA - 4 T_R \NF}{6}\;,\nonumber  \\
%\beta_1 &=& \frac{17 \CA^2 - 10 C_A T_R \NF- 6C_F T_R \NF}{6}\;, \nonumber \\
%\beta_2 &=&\frac{1}{432}
%\big( 2857 C_A^3 + 108 C_F^2 T_R N_F -1230 C_FC_A T_R N_F
%-2830 C_A^2T_RN_F \nonumber \\ &&
%+ 264 C_FT_R^2 N_F^2 + 316 C_AT_R^2N_F^2\big)\;.
%\end{eqnarray}
Eq.~(\ref{eq:running})
is solved by introducing $\Lambda$ as integration constant
with $L= \log(\mu^2/\Lambda^2)$, yielding the running coupling constant:
\begin{equation}
\alpha_s(\mu) = \frac{2\pi}{\beta_0 L}\left( 1-
\frac{\beta_1}{\beta_0^2}\, \frac{\log L}{L} + \frac{1}{\beta_0^2 L^2}\,
\left( \frac{\beta_1^2}{\beta_0^2}\left( \log^2 L - \log L - 1
\right) + \frac{\beta_2}{\beta_0}  \right) \right)\;.
\end{equation}

In terms of the running coupling $\alpha_s(\mu)$, the
NNLO (non-singlet) expression for event shape distributions therefore becomes
\begin{eqnarray}
\frac{1}{\sigma_{{\rm had}}}\, \frac{\dbox\sigma}{\dbox \Obs} (s,\mu^2,\Obs) &=&
\left(\frac{\alpha_s(\mu)}{2\pi}\right) \frac{\dbox A}{\dbox \Obs} +
\left(\frac{\alpha_s(\mu)}{2\pi}\right)^2 \left(
\frac{\dbox  B}{\dbox \Obs} + \frac{\dbox  A}{\dbox \Obs} \left[\beta_0
\log\frac{\mu^2}{s} -\frac{3}{2}\,C_F\right]\right)
\nonumber \\ &&
+ \left(\frac{\alpha_s(\mu)}{2\pi}\right)^3
\Bigg(\frac{\dbox  C}{\dbox \Obs} +  \frac{\dbox  B}{\dbox \Obs}
\left[ 2\beta_0\log\frac{\mu^2}{s}-\frac{3}{2}\,C_F\right]\nonumber\\
&&+ \frac{\dbox  A}{\dbox \Obs} \left[\beta_0^2\,\log^2\frac{\mu^2}{s}
+ \beta_1\, \log\frac{\mu^2}{s}  -3\beta_0 C_F \, \log\frac{\mu^2}{s}-K_2+\frac{9}{4}C_F^2\right]\Bigg)
\nonumber \\ &&
 + {\cal O}(\alpha_s^4)\;.
\label{eq:NNLOmu}
\end{eqnarray}
The program {\tt EERAD3} computes the perturbative coefficients
$A$, $B$ and $C$ defined in eq.~(\ref{eq:NNLOsigma0}), where the renormalisation scale
has been fixed to the centre-of-mass energy.
In order to be able to perform variations of the renormalization scale,
it is therefore sufficient to store the coefficients $A$, $B$ and $C$
in the Ntuples and apply Eq.~(\ref{eq:NNLOmu}) at the level of the Ntuple analysis.

\subsubsection{Details about the {\tt EERAD3} Ntuples}


The input file {\tt eerad3.input} contains the field {\tt nshot3\,  nshot4\,  nshot5}.
They denote the numbers of sampling points per iteration to be used by
the Monte Carlo integrator Vegas for the 3-parton, 4-parton, 5-parton channels, respectively.
The field {\tt itmax1\, itmax2} contains the number of iterations
for the ``warm up run'' (grid construction, {\tt itmax1} iterations)
and the ``production run'' (event generation and integration, {\tt itmax2} iterations).
The total number of events in each channel is then roughly given by
{\tt nshot} $\times$ {\tt itmax2}, modulo events which do not pass the
cuts.

For the implementation of this experimentation we used the same format as for the BlackHat+Sherpa NLO Ntuples~\cite{Bern:2013zja},
removing however the unnecessary information about the partonic initial states.
Figure~\ref{fig:filesizes} shows the size of the Ntuple file as a function of the number of events.
\begin{figure}
  \begin{center}
  \includegraphics[scale=0.5]{sizes.png}
  \end{center}
\caption{File size as a function of the number of events.}\label{fig:filesizes}
\end{figure}
In Table~\ref{tab:size}, we list the size of the Ntuple files
for a million events. The Ntuples contain the NNLO
results for the sum of all colour factors, i.e. {\tt icol=0}.
Further, we used {\tt y0=1d-7, iaver=0, cutvar=1d-5}.
The event numbers given in Table~\ref{tab:size} are summed over all partonic channels.


\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
run & size/Mevents [GB] & size/Mevents [GB] with mapping \\
\hline
LO  & 0.038 & 0.038  \\
NLO & 1.66& 0.56   \\
NNLO & 433.9 & 64.7\\
\hline
\end{tabular}
\end{center}
\caption{Sizes of the Ntuple files for various choices of the total number of events.\label{tab:size}}
\end{table}
The first column of Table~\ref{tab:size} shows the size of the Ntuple file if all phase-space information is recorded in the Ntuple.
An alternative strategy is to use the fact that there is a clear relationship between the kinematical information of a real phase-space point
(``real'' refers to the phase-space with the largest final state multiplicity)  and its subtractions.
Starting from one phase-space configuration for the real radiation one can get to all the kinematical configurations for the subtractions
using a fixed number of phase-space mappings. If we can enumerate these mappings and record the mapping label instead of the actual mapped momenta
we can save a significant amount of storage, at the cost of having to perform the mappings when the Ntuple file is analysed.
The second column of Table~\ref{tab:size} shows the size of an Ntuple file if the mapping label is recorded instead of the momenta for the subtractions.
However, apart from the increased CPU time to read an Ntuple file produced in this way there is another disadvantage:
the Ntuple is more tightly bound to the program that produced it, as the implementation of the mappings has to be provided along with the Ntuple file.

We should mention that the reconstruction of observables from the information contained in the
Ntuples is
only applicable to observables which are rotation-invariant. This is due to the fact that
the phase space in {\tt EERAD3} is constructed assuming rotational invariance.


\subsection{Summary and outlook}

We have produced Root Ntuple files based on the program {\tt EERAD3}, a partonic Monte Carl program  to calculate  event shapes and
jet rates in electron-positron annihilation up to NNLO.
We have found that the size of the Ntuple files needed to produce
reasonably smooth histograms is of the order of 2-3 TeraBytes.
Therefore it seems that Ntuples can be a convenient way to store NNLO results in hadronic collisions as well.

Apart from the obvious advantages of Ntuples to be able to perform
scale and PDF variations without having to run the full program,
there are a number of other aspects which make the use of Ntuples for
NNLO results additionally appealing:
\begin{itemize}
\item the results can be made available to experimentalists,
where they can apply different sets of cuts, PDFs, etc.
 without having to deal with the NNLO code
\item it is easy to change value of $\alpha_s(M_Z)$,
such that fits of  $\alpha_s$ could be readily performed.
%\item the output fits into the format of the fastNLO framework
\end{itemize}
The file sizes presented here are obtained using the EERAD3 phase-space generator that was designed to optimize the CPU time.
One can easily imagine that, if the focus was shifted to optimise the storage space, improvements for the file size could be achieved.

We are looking forward to the first NNLO results in hadronic collisions being available in the form of Ntuples.

%comments about things to be improved in the EERAD3 program:\\
%option ``NLO only'' in eerad3\_dist is not possible at the moment\\
%improve  PS generator, based od pp to dijet experience?



==> psrew_main.tex <==
\section{Reweighting the \texorpdfstring{S\protect\scalebox{0.8}{HERPA}}{SHERPA} parton shower \texorpdfstring{\protect\footnote{ E.\ Bothmann, M.\ Sch\"onherr, S.\ Schumann}}{}}
\label{sec:psrew}

\subsection{Introduction}

The last ten years of improving Monte-Carlo event generators (MCEG) enabled
quantitative predictions at an unprecedented accuracy. These developments 
led to a considerable growth in computational cost per event. This can become
limiting, as calculations must often be performed repeatedly, 
e.g.\ to assess theory uncertainties. For QCD calculations such 
re-calculations are necessary for each combination of QCD input parameters. 
Those include parton density functions (PDF), the strong coupling 
($\alpha_S$) or the renormalisation/factorisation scale. This adds up 
to $\mathcal{O}(10^3)$ re-calculations quickly. For PDF fits, the 
demand for re-calculations is even higher.

This issue is addressed by \emph{not doing the whole calculation again}.
Instead, parameter-independent bits of the calculation are stored
as weights and can then be recombined with different parameter values.
This can either be done directly for each event,
or after projecting weights to interpolation grids first,
with one grid per observable bin and dependence
structure~\cite{Carli:2010rw,Kluge:2006xs}.
PDF fitters use such interpolation grids for cross section predictions,
as the time needed for a recombination is of the order of milliseconds only.

For leading-order (LO) events, getting the \emph{parameter-indendent weight} is easy:
divide the event weight
by the PDFs $f_a f_b$ of the incoming partons
and by $\alpha_S^p$, with $p$ being the perturbative order of the process.
Then multiply with $f'_a f'_b \alpha_S'^p$ to get the new event weights
for a different set of input PDFs $f'$ and a different value of the strong 
coupling $\alpha_S'$. For the proper evaluation of these {\em variational
weights} the partonic momentum fractions $x_{1}$ and $x_{2}$ as well as
the factorisation and renormalisation scale need to be book-kept.
At next-to-leading order (NLO)
the procedure is more complicated, because of the additional scale-dependence 
of the virtual corrections and the different kinematics and initial states of the 
subtraction parts~\cite{Bern:2013zja}.

The newly added internal reweighting of \textsc{Sherpa}~\cite{Gleisberg:2008ta}
as of version 2.2.0 performs \emph{on-the-fly}
during event generation~\cite{Bothmann:2015woa}. The result for each combination is inserted into the
{\small \tt HepMC::WeightContainer} object and thus can be either saved to disk,
programmatically accessed or directly passed via the internal interface to the
{\small \tt Rivet} analysis framework~\cite{Buckley:2010ar}.
The supported event generation modes are (N)LO, (N)LO+PS (i.e. matched to a parton shower)
and MEPS@LO (i.e. merged LO matrix elements with a shower).
The recently introduced interfaces {\small\tt MCgrid}~\cite{DelDebbio:2013kxa} and
{\small\tt aMCfast}~\cite{Bertone:2014zva} on the other hand
allow for the automated creation of interpolation grids using
general MCEGs. (N)LO and (N)LO+PS are supported.

For both reweighting approaches, event generations
involving a parton shower come with a caveat:
The shower takes no part
in the reweighting procedure, and is kept as-is. Its dependences
on PDF, scale and $\alpha_S$ are thus not taken into account.
Therefore the reweighting leads to an \emph{inconsistent result},
where dependences in the hard process have been updated,
but not in the shower.
There are indications that this does not affect major parts of
phase space~\cite{Buckley:2016caq,Gieseke:2004tc}.
A more thorough study is however still missing.
We address this by presenting ongoing work to extend the internal 
\textsc{Sherpa} reweighting to include all dependences of the 
parton shower emissions, using a property of the
veto algorithm that allows for a simple multiplicative reweighting.

\subsection{Reweighting the veto algorithm}

The default shower of \textsc{Sherpa}, \textsc{Csshower} \cite{Schumann:2007mg}, 
uses the veto algorithm to
numerically integrate the Sudakov form factors
\begin{equation}
  \Delta(t_0, t_c) = e^{- \int_{t_c}^{t_0} \Gamma(t) \mathrm{d} t}\,,
\end{equation}
which give the no-branching probabilities between the starting scale
$t_0$ and the cut-off scale $t_c$.
In the veto algorithm the splitting kernels $\Gamma$ are replaced with
integrable overestimates $\hat{\Gamma}$. This is balanced by only accepting a
proposed emission with the probability $P_\mathrm{acc} = \Gamma / \hat{\Gamma}$.
A multiplicative factor in $\Gamma$ is therefore equivalent to a
multiplicative factor in $P_\mathrm{acc}$~\cite{Hoeche:2009xc}.
This observation is for example used to apply matrix element 
corrections~\cite{Hoeche:2011fd}, where the splitting kernels are replaced 
with a real-emission-like kernel $R/B$. This is done a-posteriori, i.e. the event weight is multiplied
by $(R/B)/\Gamma$. The emission itself is unchanged.
The same method is also used in the {\small\tt Vincia} parton shower to calculate
uncertainty variations for different scales, finite terms of the antenna functions,
ordering parameters and sub-leading colour corrections~\cite{Giele:2011cb}.

The emission kernels $\Gamma$ depend linearly on $\alpha_S$ and
on a ratio of PDF values $f_a(x/z)/f_b(x)$\footnote{The exact definition of
the flavours $a$, $b$ and the momentum fractions $x$, $x/z$ depend on the
dipole configuration of the emission. There is no PDF dependence in the case
of dipoles that consist only of final-state partons.}.
A change of PDFs $f \rightarrow f'$ and the strong coupling
$\alpha_S \rightarrow \alpha_S'$
is equivalent to modifying the emission probability
accordingly\footnote{Both $\alpha_S$ and $f$ depend on the
emission scale. Although the emission scales can not be
reweighted themselves using the presented method, the functional
form of these dependences can be changed.}:
\begin{equation}
  P_\mathrm{acc} \rightarrow q\,P_\mathrm{acc}\,,\qquad
  q \equiv \frac{\alpha_S'}{\alpha_S} \cdot
  \frac{f'_a(x/z)/f'_b(x)}{f_a(x/z)/f_b(x)}\,,
\end{equation}
i.e. we need to multiply the event weight for each accepted emission by the 
corresponding $q$ in order to reweight the event with a new choice of PDFs.
For the rejected emissions we obtain
\begin{equation}
  P_\mathrm{rej} = 1 - P_\mathrm{acc} \rightarrow 1 - q P_\mathrm{acc}
  = \left[ 1 + \left( 1 - q \right) \frac{P_\mathrm{acc}}{1 - P_\mathrm{acc}}
    \right]\,P_\mathrm{rej}\,,
\end{equation}
so for each of those we need to multiply the event weight with the expression
in square brackets.

Our current implementation supports PDF and $\alpha_S$ reweighting of parton shower emissions for
both LO+PS and NLO+PS events.
One can choose a maximum number
of reweighted emissions per event.
This is useful because some observables are
sensitive only to the first few emissions.
The reduced amount of reweighting per event then
allows for faster event generations.


\subsection{Validation}

We present a selection of plots to validate our implementation.
All contain comparisons between ``dedicated'' and ``reweighted'' results.
The ``dedicated'' results are produced through normal runs for the varied
input parameters, whereas the ``reweighted'' ones are obtained by reweightings
from a run with a central parameter choice.
The reweighting is done for the matrix element exclusively (``ME''),
including all parton shower emissions (``ME+PS'') or just
the first emission (``ME+PS(1st em.)'').

In Fig.~\ref{psrew_fig:appl}, we present uncertainty bands for PDF and 
$\alpha_S$ variations. The left-hand plot features a 
{\small\tt CT14nlo}~\cite{Dulat:2015mca} PDF error band for the $W$-boson
transverse momentum distribution in $W$ production
at the LHC at NLO+PS. The band is a combination of the central member and 56
Hessian eigenvector members. So for the ``dedicated'' band,
57 independent event generation runs had to be performed,
whereas each of the reweighting bands is generated by
a single run.\footnote{We are yet to do a detailed timing
study (and to optimise the code), but for the case of doing 57 variations
and reweighting the ME and up to one parton shower emission,
the run took about a factor of 6 longer than a run
without any reweighting.
% NOTE: For reweighting all emissions, I've found a factor of ~13
Comparing the time needed to generate the entire error band,
the reweighting run thus needed one order of magnitude
less than the combination of dedicated runs.}

A few observations can be made for the $W$ $p_\perp$ plot: (i) For
$p_\perp < 10$ GeV, solely reweighting the ME underestimates 
the error found with the dedicated calculation by about 4\,\% 
in both directions. The ME+PS reweighting is able to reproduce the error.
(ii) For $p_\perp$ values between 20\,GeV and the $W$~mass,
the ME reweighting \emph{overestimates} the positive error slightly,
by about 1\,\%. Again, the ME+PS reweighting correctly
reproduces the error.
(iii) The reweighted bands are much smoother because the prediction
for each PDF member shares the statistics of the central run.
Unfortunately there is no way to guarantee this for the dedicated
runs when varying input parameters of the parton shower,
which makes closure tests between reweighting and dedicated runs a
statistical exercise.

The right-hand plot in Fig.~\ref{psrew_fig:appl}
contains a band for an $\alpha_S$ variation for the thrust
observable for $e^+e^- \to q\bar{q}$ at LEP at LO+PS.
The variations considered around the central values of 
$\alpha_S(m_Z)=0.120$ include $\alpha_S(m_Z)=0.108$ and 
$\alpha_S(m_Z)=0.128$. The running of $\alpha_S$ is evaluated 
at the one-loop order. The plot shows the envelope for the three values.
The reweighted band is obtained by reweighting
all emissions in the run with the central $\alpha_S$ value.
It reproduces the dedicated band within statistical errors.
For this we note that the variance of the reweighted prediction
increases. In some bins, the sum of squared weights is a factor
of 100 higher compared to the dedicated result.

Jet resolutions are sensitive to the specifics of parton shower emissions,
which is why we have in Fig.~\ref{psrew_fig:nrew} a series of closure tests
for this observable for $W$-boson production at the LHC at LO+PS.
The reweightings are done from the central {\small\tt CT14}
to the central {\small\tt MMHT2014} set~\cite{Harland-Lang:2014zoa}.
The maximum number of shower emissions
being reweighted is varied between 0, 1 and $\infty$.
The corresponding reweighted
predictions are compared to the dedicated {\small\tt MMHT2014} result.
This is done for the $0\to1$ and for the $3\to4$ jet resolution.
We observe deviations for the ME-only reweighting prediction of about $\pm2\,\%$.
The 1-emission-reweighting fixes the deviation for $d_{01} > 10$ GeV, but can not
fix the deviations elsewhere. The all-emissions-reweighting is perfect within statistics
for all bins of both jet resolutions.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\textwidth]{psrew_W_pT}
\includegraphics[width=0.49\textwidth]{psrew_Thrust}
\caption{A PDF variation for the $W$-boson $p_\perp$ distribution at the LHC 
  at NLO+PS (left) and an $\alpha_S$ variation for the Thrust for $q\bar{q}$ 
  production at LEP at LO+PS (right). Predictions generated by single 
  reweighting runs (``rew'd'') are compared to predictions from dedicated runs.}
\label{psrew_fig:appl}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\textwidth]{psrew_log10_d_01}
\includegraphics[width=0.49\textwidth]{psrew_log10_d_34}
\caption{Predictions for jet resolutions for $W$-boson productions at the LHC 
  at LO+PS. Results from reweighting runs {\small\tt CT14} $\to$ {\small\tt MMHT2014} 
  PDF are compared to the dedicated result for direct use of the {\small\tt MMHT2014} 
  PDF.}
\label{psrew_fig:nrew}  
\end{figure}

\subsection{Conclusions}

We have presented the extension of the internal reweighting of \textsc{Sherpa}
to include the $\alpha_S$ and PDF dependences of parton shower emissions.
It has been shown that the ME-only reweighting has shortcomings compared to the newly
implemented full reweighting.
We did this by comparing theory uncertainty bands generated by reweighting runs
with dedicated calculations for $\alpha_S$ and PDF variations at LO+PS and (N)LO+PS.
Now with the support for these input parameters in place, the next step is to
allow for varying the scales at which $\alpha_S$ and the PDFs are evaluated
for a given emission. This is different from varying the actual emission scale
(e.g.\ indirectly by choosing a new starting scale), which is not covered
by the presented reweighting method.

The full direct reweighting for parton showers
will leave us with a complete picture of
how to reweight when all information is still available.
This will help us when bringing parton shower reweighting
also to grids, where individual event information is \emph{not} available.
For this we are considering an approximate approach.
Such shower-aware grids would allow for including more data in PDF fits,
namely data that is currently omitted because its theoretical prediction
is sensitive to higher-order corrections.

\subsection*{Acknowledgements}
We acknowledge financial support from BMBF under contract 05H15MGCAA, 
the Swiss National Foundation (SNF) under contract PP00P2--128552 and 
from the EU MCnetITN research network funded under Framework Programme 
7 contract PITN--GA--2012--315877.



==> psuncertainties_main.tex <==
\section{Towards parton shower variations \texorpdfstring{\protect\footnote{ S.\ H\"oche, A.\ Jueid, G.\ Nail, S.\ Pl\"atzer,  M.\ Sch\"onherr, A.\ Si\'odmok, P.\ Skands, D.\ Soper, K.\ Zapp}}{}}
\input{psuncertainties_intro}
\input{psuncertainties_tools}
\input{psuncertainties_results}
\input{psuncertainties_conclusions}

